RoboCoder: Robotic Learning from Basic Skills to General Tasks with Large Language Models

The emergence of Large Language Models (LLMs) has improved the prospects for robotic tasks. However, existing benchmarks are still limited to single tasks with limited generalization capabilities. In this work, we introduce a comprehensive benchmark and an autonomous learning framework, RoboCoder aimed at enhancing the generalization capabilities of robots in complex environments. Unlike traditional methods that focus on single-task learning, our research emphasizes the development of a general-purpose robotic coding algorithm that enables robots to leverage basic skills to tackle increasingly complex tasks. The newly proposed benchmark consists of 80 manually designed tasks across 7 distinct entities, testing the models' ability to learn from minimal initial mastery. Initial testing revealed that even advanced models like GPT-4 could only achieve a 47% pass rate in three-shot scenarios with humanoid entities. To address these limitations, the RoboCoder framework integrates Large Language Models (LLMs) with a dynamic learning system that uses real-time environmental feedback to continuously update and refine action codes. This adaptive method showed a remarkable improvement, achieving a 36% relative improvement. Our codes will be released.

==> tables/dofs.tex <==
\begin{table}
\centering
\footnotesize
\setlength{\tabcolsep}{1.5mm}
\caption{Degrees of Freedom (DOFs) for Joint Movements: 21 indices representing joint positions and their corresponding movement directions.}
\label{tab:joint_indices}
\begin{tabular}{@{}clll|clll@{}}
\toprule
\textbf{Index} & \textbf{Joint} & \textbf{Lower} & \textbf{Upper} & \textbf{Index} & \textbf{Joint} & \textbf{Lower} & \textbf{Upper} \\ 
\midrule
0 & Abdomen Z & Clockwise & Anticlockwise & 10 & Left Hip Z & Anticlockwise & Clockwise \\
1 & Abdomen Y & Forward & Backward & 11 & Left Hip Y & Forward & Backward \\
2 & Abdomen X & Left & Right & 12 & Left Knee & Backward & Forward \\
3 & Right Hip X & Right & Left & 13 & Left Ankle Y & Forward & Backward \\
4 & Right Hip Z & Clockwise & Anticlockwise & 14 & Left Ankle X & Right & Left \\
5 & Right Hip Y & Forward & Backward & 15 & Right Shoulder1 & Left & Right \\
6 & Right Knee & Backward & Forward & 16 & Right Shoulder2 & Backward & Forward \\
7 & Right Ankle Y & Forward & Backward & 17 & Right Elbow & Forward & Backward \\
8 & Right Ankle X & Right & Left & 18 & Left Shoulder1 & Right & Left \\
9 & Left Hip X & Left & Right & 19 & Left Shoulder2 & Backward & Forward \\
\multicolumn{4}{c|}{} & 20 & Left Elbow & Forward & Backward \\
\bottomrule
\end{tabular}
\label{tab:dofs}
\end{table}


==> tables/performance.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Previous results: more models with table
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\iffalse
\begin{figure}[t]
    \centering
    \begin{minipage}{0.48\textwidth}
        \centering
        \setlength{\tabcolsep}{0.8mm}
        \captionof{table}{Performance of SOTA coding models.}
        \begin{tabular}{@{}lcc@{}}
        \toprule
        \textbf{Method} & \textbf{Baseline} & \textbf{RoboCoder} \\ \midrule
        StarCoder-15B & 16.98 & 24.53 \textcolor{teal}{\scriptsize (+7.55)} \\
        WizardCoder-15B & 26.42 & 32.08 \textcolor{teal}{\scriptsize (+5.66)} \\
        CodeLlama-Instruct-13b & 26.42 & 33.96 \textcolor{teal}{\scriptsize (+7.54)} \\
        CodeLlama-Instruct-34b & 32.08 & 47.17 \textcolor{teal}{\scriptsize (+15.09)} \\
        GPT3.5 & 54.72 & 73.58 \textcolor{teal}{\scriptsize (+18.86)} \\
        GPT4 & 55.77 & 75.00 \textcolor{teal}{\scriptsize (+19.23)} \\
        \iffalse
        StarCoder-15B~\cite{starcoder} & 16.98 & 24.53 \textcolor{teal}{\scriptsize (+7.55)} \\
        WizardCoder-15B~\cite{wizardcoder} & 26.42 & 32.08 \textcolor{teal}{\scriptsize (+5.66)} \\
        CodeLlama-Instruct-13b~\cite{codellama} & 26.42 & 33.96 \textcolor{teal}{\scriptsize (+7.54)} \\
        CodeLlama-Instruct-34b~\cite{codellama} & 32.08 & 47.17 \textcolor{teal}{\scriptsize (+15.09)} \\
        GPT3.5~\cite{gpt3.5} & 54.72 & 73.58 \textcolor{teal}{\scriptsize (+18.86)} \\
        GPT4~\cite{openai2023gpt4} & 55.77 & 75.00 \textcolor{teal}{\scriptsize (+19.23)} \\
        \fi
        \bottomrule
        \end{tabular}
        \label{tab:performance}
    \end{minipage}
    \hfill
    \begin{minipage}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth, trim=0 0 0 0, clip]{figures/performance.pdf}
        \captionof{figure}{Performance across iterations.} % , including StarCoder-15B, WizardCoder-15B, CodeLLaMA-Instruct-13B and 15B, GPT3.5, and GPT4.
        \label{fig:performance}
    \end{minipage}
\end{figure}
\fi
